Homotopy Type Theory: Univalent Foundations of Mathematics

Homotopy type theory is a new branch of mathematics, based on a recently discovered connection between homotopy theory and type theory, which brings new ideas into the very foundation of mathematics. On the one hand, Voevodsky's subtle and beautiful "univalence axiom" implies that isomorphic structures can be identified. On the other hand, "higher inductive types" provide direct, logical descriptions of some of the basic spaces and constructions of homotopy theory. Both are impossible to capture directly in classical set-theoretic foundations, but when combined in homotopy type theory, they permit an entirely new kind of "logic of homotopy types". This suggests a new conception of foundations of mathematics, with intrinsic homotopical content, an "invariant" conception of the objects of mathematics -- and convenient machine implementations, which can serve as a practical aid to the working mathematician. This book is intended as a first systematic exposition of the basics of the resulting "Univalent Foundations" program, and a collection of examples of this new style of reasoning -- but without requiring the reader to know or learn any formal logic, or to use any computer proof assistant.

==> opt-a4.tex <==
%%% FORMATTING OPTIONS FOR A4 SIZE
%%% This file gets included by the hott-xxx.tex files.

% MACROS FOR FINE TUNING
\newcommand{\narrowbreak}{}
\newcommand{\narrowequation}[1]{$#1$}
\newenvironment{narrowmultline}{\csname equation\endcsname}{\csname endequation\endcsname}
\newenvironment{narrowmultline*}{\csname equation*\endcsname}{\csname endequation*\endcsname}

% FONTS
\def\OPTfontsize{11pt}        % Font size

% PAGE FORMAT
%
% These settings are for A4 format
\def\OPTpagesize{210mm,297mm} % Page size
\def\OPTtopmargin{1in}        % Margin at the top of the page
\def\OPTbottommargin{1in}     % Margin at the bottom of the page
\def\OPTbindingoffset{0.35in} % Extra offset on the inner side

% Tweak the margins so the textwidth is the same as in the letter version
%
% The letter margins are:
%
% \def\OPTinnermargin{0.75in}   % Margin on the inner side of the page
% \def\OPToutermargin{1.0in}    % Margin on the outer side of the page
%
% and half the difference between 8.5in and 210mm is 2.95mm

\newskip\innermarginskip
\innermarginskip=0.75in
\advance\innermarginskip by -2.95mm
\edef\OPTinnermargin{\the\innermarginskip}

\newskip\outermarginskip
\outermarginskip=1.0in
\advance\outermarginskip by -2.95mm
\edef\OPToutermargin{\the\outermarginskip}

% FORMATTING OF COVER PAGE
\def\OPTcoverwidth{8.45in}    % width of text on cover page
\def\OPTcoverheight{10.95in}  % height of text on cover page
\def\OPTtopskip{43pt}         % Skip at top of cover and back page (with units)
\def\OPTbotskip{43pt}         % Skip at bottom of cover and back page (with units)
\def\OPTcovertitlefont{74.5}  % Size of title font (no unit, pt assumed)
\def\OPTcovertitleskip{24pt}  % Skip between title and subtitle (with units)
\def\OPTcoversubtitlefont{27} % Size of subtitle font (no unit, pt assumed)
\def\OPTcoverauthorfont{22}   % Size of author font (no unit, pt assumed)
\def\OPTcoverauthorskip{8pt}  % Skip betewen first and second line of author (with units)

% FORMATTING OF BACK COVER PAGE
\def\OPTbacktitlefont{\LARGE} % Size of "From the introduction" and "Get this book ..."
\def\OPTbackfont{\large}      % Size of text font

% FORMATTING OF BASTARD TITLE, IF PRESENT
% (see opt-no-bastard.tex and opt-bastard.tex)
\def\OPTbastardtitlefont{22}
\def\OPTbastardsubtitlefont{15}
\def\OPTbastardwidth{0.40\textwidth} % Width of bastard title
\def\OPTbastardtitleskip{8pt}

% FORMATTING OF TITLE PAGE
\def\OPTtitletitlefont{37}    % Size of title font (no unit, pt assumed)
\def\OPTtitletitleskip{10pt}  % Skip between title and subtitle (with units)
\def\OPTtitlesubtitlefont{25} % Size of subtitle font (no unit, pt assumed)
\def\OPTtitlewidth{0.65\textwidth} % Width of title
\def\OPTtitleskip{30pt}       % Skip between title and author (with units)
\def\OPTtitleauthorfont{18}   % Size of author font (no unit, pt assumed)
\def\OPTtitleauthorskip{6pt}  % Skip betewen first and second line of author (with units)

% FORMATTING OF PART PAGE
\def\OPTpartfont{40}          % Size of "Part X" (without unit, pt assumed)
\def\OPTpartskip{20pt}        % Skip between Part and title (with unit)
\def\OPTparttitlefont{60}     % Size of part title (without unit, pt assumed)

% FORMATTING OF CHAPTER TITLE
\def\OPTchapterfont{23}       % Size of "Chapter X"
\def\OPTchapterskip{20pt}     % Skip between Chapter and title
\def\OPTchaptertitlefont{35}  % Size of chapter title

% FORMATTING OF PREFACE
\def\OPTprefacecols{3}        % Number of columns when listing people in Preface

% GETTING RID OF THE WIDOW ON PAGE 2 IN LETTER FORMAT
\def\OPTwidow{\enlargethispage{\baselineskip}}

% FORMATTING OF TABLE 1 IN INTRODUCTION
\def\OPTsmalltable{}

% FORMATTING OF TABLE 8.1 OF HOMOTOPY GROUPS OF SPHERES
\newcommand{\OPTspherescolwidth}{30pt}

% FORMATTING THE BIBLIOGRAPHY
\newcommand{\OPTbibliographyfont}{\small}

% FORMATTING OF INDEX
\newcommand{\OPTindexfont}{\small}      % size of font in the index
\newcommand{\OPTindexcolumnsep}{20.0pt} % column separation in index (default is 10.0pt)


==> opt-bastard.tex <==
% Include a bastard title
\newif\ifOPTbastard
\OPTbastardtrue


==> opt-black-white.tex <==
% Options for black & white book

% BACKGROUND OF COVER PAGE
\def\OPTcovercolor{0,0,0,0}
\def\OPTcovertextcolor{0,0,0,1}

% COVER IMAGE
\def\OPTlofrontimage{cover-lores-front-bw.png}
\def\OPTlobackimage{cover-lores-back-bw.png}
\def\OPThifrontimage{cover-hires-front-bw.png}
\def\OPThibackimage{cover-hires-back-bw.png}

% LINK COLORS
\def\OPTlinkcolor{0,0,0}       % RGB components for clickable links

% PICTURE COLORS
\def\OPTblue{black}
\def\OPTred{black}
\def\OPTpurple{black}

% COLORS FOR TABLE 8.1
\def\OPTcolormodel{gray}
\def\OPTcolxA{0.95}
\def\OPTcolxB{0.75}
\def\OPTcolxC{0.85}
\def\OPTcolxD{0.95}
\def\OPTcolxE{0.75}
\def\OPTcolxF{0.85}
\def\OPTcolxG{0.95}
\def\OPTcolxH{0.75}
\def\OPTcolxI{0.85}
\def\OPTcolxJ{0.95}
\def\OPTcolxK{0.75}
\def\OPTcolxL{0.85}
\def\OPTcolxM{0.95}


==> opt-ebook.tex <==
%%% FORMATTING OPTIONS FOR EBOOK SIZE.
%%$ THIS IS ACTUALLY USTRADE SIZE WITH SMALL MARGINS.
%%% This file gets included by the hott-xxx.tex files.

% MACROS FOR FINE TUNING
\newcommand{\narrowbreak}{\\}
\newcommand{\narrowequation}[1]{\begin{equation*}#1\end{equation*}}
\newenvironment{narrowmultline*}{\csname multline*\endcsname}{\csname endmultline*\endcsname}
\newenvironment{narrowmultline}{\csname multline\endcsname}{\csname endmultline\endcsname}

% FONTS
\def\OPTfontsize{10pt}        % Font size
\delimiterfactor=800

% PAGE FORMAT
%
% These settings are for letter format
\def\OPTpagesize{4.8in,7.9in}   % Page size
\def\OPTtopmargin{0.2in}     % Margin at the top of the page
\def\OPTbottommargin{0.2in}  % Margin at the bottom of the page
\def\OPTinnermargin{0.2in}    % Margin on the inner side of the page
\def\OPTbindingoffset{0.0in} % Extra offset on the inner side
\def\OPToutermargin{0.2in}   % Margin on the outer side of the page

% FORMATTING OF COVER PAGE
\def\OPTcoverwidth{4.75in}    % width of text on cover page
\def\OPTcoverheight{7.85in}  % height of text on cover page
\def\OPTtopskip{35pt}         % Skip at top of cover and back page (with units)
\def\OPTbotskip{35pt}         % Skip at bottom of cover and back page (with units)
\def\OPTcovertitlefont{48}    % Size of title font (no unit, pt assumed)
\def\OPTcoverspinefont{22}    % Size of title font on the book spine (no unit, pt assumed)
\def\OPTcovertitleskip{18pt}  % Skip between title and subtitle (with units)
\def\OPTcoversubtitlefont{18} % Size of subtitle font (no unit, pt assumed)
\def\OPTcoverauthorfont{14}   % Size of author font (no unit, pt assumed)
\def\OPTcoverauthorskip{6pt}  % Skip betewen first and second line of author (with units)

% FORMATTING OF BACK COVER PAGE
\def\OPTbacktitlefont{\large} % Size of "From the introduction" and "Get this book ..."
\def\OPTbackfont{\small} % Size of text font

% FORMATTING OF BASTARD TITLE, IF PRESENT
% (see opt-no-bastard.tex and opt-bastard.tex)
\def\OPTbastardtitlefont{17}
\def\OPTbastardsubtitlefont{11}
\def\OPTbastardwidth{0.42\textwidth} % Width of bastard title
\def\OPTbastardtitleskip{6pt}

% FORMATTING OF TITLE PAGE
\def\OPTtitletitlefont{22}    % Size of title font (no unit, pt assumed)
\def\OPTtitletitleskip{7pt}   % Skip between title and subtitle (with units)
\def\OPTtitlesubtitlefont{15} % Size of subtitle font (no unit, pt assumed)
\def\OPTtitlewidth{0.65\textwidth} % Width of title
\def\OPTtitleskip{21pt}       % Skip between title and author (with units)
\def\OPTtitleauthorfont{13}   % Size of author font (no unit, pt assumed)
\def\OPTtitleauthorskip{4pt}  % Skip betewen first and second line of author (with units)

% PART FONTS
\def\OPTpartfont{28}          % Size of "Part X" (without unit, pt assumed)
\def\OPTpartskip{14pt}        % Skip between Part and title (with unit)
\def\OPTparttitlefont{42}     % Size of part title (without unit, pt assumed)

% FORMATTING OF CHAPTER TITLE
\def\OPTchapterfont{20}       % Size of "Chapter X" (without unit, pt assumed)
\def\OPTchapterskip{14pt}     % Skip between Chapter and title (with unit)
\def\OPTchaptertitlefont{24}  % Size of chapter title (without unit, pt assumed)

% FORMATTING OF PREFACE
\def\OPTprefacecols{2}        % Number of columns when listing people in Preface

% GETTING RID OF THE WIDOW ON PAGE 2 IN LETTER FORMAT
\def\OPTwidow{}

% FORMATTING OF TABLE 1 IN INTRODUCTION
\def\OPTsmalltable{\small}

% FORMATTING OF TABLE 8.1 OF HOMOTOPY GROUPS OF SPHERES
\newcommand{\OPTspherescolwidth}{20pt}

% FORMATTING THE BIBLIOGRAPHY
\newcommand{\OPTbibliographyfont}{\small}

% FORMATTING OF INDEX
\newcommand{\OPTindexfont}{\footnotesize} % size of font in the index
\newcommand{\OPTindexcolumnsep}{15.0pt}   % column separation in index (default is 10.0pt)


==> opt-no-cover.tex <==
% Do not include cover
\newif\ifOPTcover
\OPTcoverfalse


==> opt-ustrade.tex <==
%%% FORMATTING OPTIONS FOR USTRADE SIZE
%%% This file gets included by the hott-xxx.tex files.

% MACROS FOR FINE TUNING
\newcommand{\narrowbreak}{\\}
\newcommand{\narrowequation}[1]{\begin{equation*}#1\end{equation*}}
\newenvironment{narrowmultline*}{\csname multline*\endcsname}{\csname endmultline*\endcsname}
\newenvironment{narrowmultline}{\csname multline\endcsname}{\csname endmultline\endcsname}

% FONTS
\def\OPTfontsize{10pt}        % Font size
\delimiterfactor=800

% PAGE FORMAT
%
% These settings are for letter format
\def\OPTpagesize{6in,9in}     % Page size
\def\OPTtopmargin{0.75in}     % Margin at the top of the page
\def\OPTbottommargin{0.75in}  % Margin at the bottom of the page
\def\OPTinnermargin{0.5in}    % Margin on the inner side of the page
\def\OPTbindingoffset{0.35in} % Extra offset on the inner side
\def\OPToutermargin{0.75in}   % Margin on the outer side of the page

% FORMATTING OF COVER PAGE
%\def\OPTcoverwidth{8.45in}    % width of text on cover page, not used for US trade
%\def\OPTcoverheight{10.95in}  % height of text on cover page
\def\OPTtopskip{35pt}         % Skip at top of cover and back page (with units)
\def\OPTbotskip{35pt}         % Skip at bottom of cover and back page (with units)
\def\OPTcovertitlefont{61}    % Size of title font (no unit, pt assumed)
\def\OPTcoverspinefont{32}    % Size of title font on the book spine (no unit, pt assumed)
\def\OPTcovertitleskip{20pt}  % Skip between title and subtitle (with units)
\def\OPTcoversubtitlefont{22} % Size of subtitle font (no unit, pt assumed)
\def\OPTcoverauthorfont{18}   % Size of author font (no unit, pt assumed)
\def\OPTcoverauthorskip{6pt}  % Skip betewen first and second line of author (with units)

% FORMATTING OF BACK COVER PAGE
\def\OPTbacktitlefont{\Large} % Size of "From the introduction" and "Get this book ..."
\def\OPTbackfont{\normalsize} % Size of text font

% FORMATTING OF BASTARD TITLE, IF PRESENT
% (see opt-no-bastard.tex and opt-bastard.tex)
\def\OPTbastardtitlefont{17}
\def\OPTbastardsubtitlefont{11}
\def\OPTbastardwidth{0.42\textwidth} % Width of bastard title
\def\OPTbastardtitleskip{6pt}

% FORMATTING OF TITLE PAGE
\def\OPTtitletitlefont{26}    % Size of title font (no unit, pt assumed)
\def\OPTtitletitleskip{7pt}   % Skip between title and subtitle (with units)
\def\OPTtitlesubtitlefont{17} % Size of subtitle font (no unit, pt assumed)
\def\OPTtitlewidth{0.65\textwidth} % Width of title
\def\OPTtitleskip{21pt}       % Skip between title and author (with units)
\def\OPTtitleauthorfont{13}   % Size of author font (no unit, pt assumed)
\def\OPTtitleauthorskip{4pt}  % Skip betewen first and second line of author (with units)

% PART FONTS
\def\OPTpartfont{28}          % Size of "Part X" (without unit, pt assumed)
\def\OPTpartskip{14pt}        % Skip between Part and title (with unit)
\def\OPTparttitlefont{42}     % Size of part title (without unit, pt assumed)

% FORMATTING OF CHAPTER TITLE
\def\OPTchapterfont{20}       % Size of "Chapter X" (without unit, pt assumed)
\def\OPTchapterskip{14pt}     % Skip between Chapter and title (with unit)
\def\OPTchaptertitlefont{24}  % Size of chapter title (without unit, pt assumed)

% FORMATTING OF PREFACE
\def\OPTprefacecols{2}        % Number of columns when listing people in Preface

% GETTING RID OF THE WIDOW ON PAGE 2 IN LETTER FORMAT
\def\OPTwidow{}

% FORMATTING OF TABLE 1 IN INTRODUCTION
\def\OPTsmalltable{\small}

% FORMATTING OF TABLE 8.1 OF HOMOTOPY GROUPS OF SPHERES
\newcommand{\OPTspherescolwidth}{20pt}

% FORMATTING THE BIBLIOGRAPHY
\newcommand{\OPTbibliographyfont}{\small}

% FORMATTING OF INDEX
\newcommand{\OPTindexfont}{\footnotesize} % size of font in the index
\newcommand{\OPTindexcolumnsep}{15.0pt}   % column separation in index (default is 10.0pt)

